ThinkDial: An Open Recipe for Controlling Reasoning Effort in Large Language Models

Large language models (LLMs) with chain-of-thought reasoning have demonstrated remarkable problem-solving capabilities, but controlling their computational effort remains a significant challenge for practical deployment. Recent proprietary systems like OpenAI's gpt-oss series have introduced discrete operational modes for intuitive reasoning control, but the open-source community has largely failed to achieve such capabilities. In this paper, we introduce ThinkDial, the first open-recipe end-to-end framework that successfully implements gpt-oss-style controllable reasoning through discrete operational modes. Our system enables seamless switching between three distinct reasoning regimes: High mode (full reasoning capability), Medium mode (50 percent token reduction with <10 percent performance degradation), and Low mode (75 percent token reduction with <15 percent performance degradation). We achieve this through an end-to-end training paradigm that integrates budget-mode control throughout the entire pipeline: budget-mode supervised fine-tuning that embeds controllable reasoning capabilities directly into the learning process, and two-phase budget-aware reinforcement learning with adaptive reward shaping. Extensive experiments demonstrate that ThinkDial achieves target compression-performance trade-offs with clear response length reductions while maintaining performance thresholds. The framework also exhibits strong generalization capabilities on out-of-distribution tasks.

==> table/parameter.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lc}
\toprule
\textbf{Parameter} & \textbf{Value} \\
\midrule
$r_{\text{medium}}$ & 0.5 \\
$r_{\text{low}}$ & 0.25 \\
$\alpha_{\text{high}}$ & 0.0 \\
$\alpha_{\text{medium}}$ & 0.5 \\
$\alpha_{\text{low}}$ & 1.0 \\
$\tau_{\text{medium}}$ & 0.65 \\
$\tau_{\text{low}}$ & 0.4 \\
$G$ & 8 \\
$N$ & 2 \\
\bottomrule
\end{tabular}
\caption{Hyperparameter settings for our controllable reasoning framework.}
\label{tab:hyperparams}
\end{table}
